Surface defects, flavored modular differential equations and modularity

Every 4d $\mathcal{N} = 2$ SCFT $\mathcal{T}$ corresponds to an associated VOA $\mathbb{V}(\mathcal{T})$, which is in general non-rational with a more involved representation theory. Null states in $\mathbb{V}(\mathcal{T})$ can give rise to non-trivial flavored modular differential equations, which must be satisfied by the refined/flavored character of all the $\mathbb{V}(\mathcal{T})$-modules. Taking some $A_1$ theories $\mathcal{T}_{g,n}$ of class-$\mathcal{S}$ as examples, we construct the flavored modular differential equations satisfied by the Schur index. We show that three types of surface defect indices give rise to common solutions to these differential equations, and therefore are sources of $\mathbb{V}(\mathcal{T})$-module characters. These equations transform almost covariantly under modular transformations, ensuring the presence of logarithmic solutions which may correspond to characters of logarithmic modules.

==> appendices/monodromy.tex <==
%!TEX root = ../defectIndexAndMDE.tex

\section{Monodromy}\label{app:monodromy}

\subsection{\texorpdfstring{$\mathfrak{so}(8)_{-2}$}{}}

We can solve the equation (\ref{unflavored-MDE-I04}) by rewriting it in terms of $\lambda\left(\tau\right)=\frac{\vartheta_2(\tau)^4}{\vartheta_3(\tau)^4}$, and transform it into an ODE as follows:
\begin{align}
\frac{1}{4}\left(\lambda-1\right)^2D^2_{\lambda}\chi\left(\lambda\right)+\frac{1}{12}\left(\lambda^2-1\right)D_{\lambda}\chi(\lambda)-\frac{35}{144}\left(\lambda^2-\lambda+1\right)\chi(\lambda)=0
\end{align}
Let $\chi\left(\lambda\right)=\left(1-\lambda\right)^{-5/6}\phi(\lambda)$, then function $\phi\left(\lambda\right)$ is solution of the following generalized hypergeometric equations:
\begin{align}
\left(D_{\lambda}-\beta_1\right)\left(D_{\lambda}-\beta_2\right)\phi\left(\lambda\right)-\lambda\left(D_{\lambda}+1-\alpha_1\right)\left(D_\lambda+1-\alpha_2\right)\phi(\lambda)=0
\end{align}
the parameters are $\alpha_1=\frac{2}{3}$, $\alpha_2=\frac{8}{3}$, $\beta_1=\frac{7}{6}$, $\beta_2=-\frac{5}{6}$. There are two linear independent solutions for this GHE:
\begin{align}
&\phi_0\left(\lambda\right)=\lambda^{\frac{7}{6}}{}_2F_1\left(\frac{3}{2},-\frac{1}{2};3;\lambda\right)\\
&\phi_1\left(\lambda\right)=G^{2,0}_{2,2}\left(\lambda\right|\left.\begin{array}{cc}
	\frac{2}{3} & \frac{8}{3} \\
	\frac{7}{6} & -\frac{5}{6}
\end{array}\right)
\end{align}
From the integral representation:
\begin{align}
{}_2F_1\left(\frac{3}{2},-\frac{1}{2};3;\lambda\right)=\frac{\Gamma\left(3\right)}{\Gamma\left(\frac{3}{2}\right)\Gamma\left(-\frac{1}{2}\right)}\frac{1}{2\pi i}\int_L\frac{\Gamma\left(\frac{3}{2}+s\right)\Gamma\left(-\frac{1}{2}+s\right)}{\Gamma\left(3+s\right)}\Gamma\left(-s\right)\left(-\lambda\right)^s ds
\end{align}
The integrated function has the following two sets of poles:$s=\frac{1}{2}$, $s=-\frac{1}{2}$, $s=-\frac{3}{2}$, $s=-\frac{5}{2}$ .... and $s=0$, $s=1$, $s=2$.... The former set of poles are arranged at the left hand side of contour $L$, the latter is on the right hand side. To obtain its Taylor expansion within $|\lambda|<1$, we pick up the residues of the poles at the right hand side of $L$, and have:
\begin{align}
{}_2F_1\left(\frac{3}{2},-\frac{1}{2};3;\lambda\right)=-\frac{2}{\pi}\sum_{n\geq 0}\frac{\Gamma\left(\frac{3}{2}+n\right)\Gamma\left(n-\frac{1}{2}\right)}{n!\Gamma\left(n+3\right)}\lambda^n\qquad |\lambda|<1
\end{align}
To obtain its Laurent expansion when $|\lambda|>1$, we simply pick up the residues of poles at the left hand side of contour $L$:
\begin{align}
&{}_2 F_1\left(\frac{3}{2},-\frac{1}{2};3;\lambda\right)=\frac{32}{15\pi}\left(-\lambda\right)^{\frac{1}{2}}+\frac{8}{3\pi}\left(-\lambda\right)^{-\frac{1}{2}}-\frac{2}{\pi}\sum_{n\geq 0}\frac{(-)^{n+1}}{\pi}\frac{\left(-\lambda\right)^{-\frac{3}{2}-n}\Gamma\left(\frac{3}{2}+n\right)\Gamma\left(n-\frac{1}{2}\right)}{n!\Gamma\left(n+3\right)}\notag\\
&\left(A_n+A_{n+2}-\psi\left(\frac{3}{2}+n\right)-\psi\left(\frac{3}{2}-n\right)+\ln\left(-\lambda\right)\right)\qquad |\lambda|>1
\end{align}
If we set $\left(-\right)=e^{\pi i}$, $\ln(-\lambda)=\ln\lambda+\pi i$, we have:
\begin{align}
&{}_2 F_1\left(\frac{3}{2},-\frac{1}{2};3;\lambda\right)=\frac{32 i}{15\pi}\left(\lambda\right)^{\frac{1}{2}}-\frac{8 i}{3\pi}\left(\lambda\right)^{-\frac{1}{2}}+\frac{2 i}{\pi^2}\sum_{n\geq 0}\frac{\Gamma\left(\frac{3}{2}+n\right)\Gamma\left(n-\frac{1}{2}\right)}{n!\Gamma\left(n+3\right)}\lambda^{-\frac{3}{2}-n}\notag\\
&\left(A_n+A_{n+2}-\psi\left(\frac{3}{2}+n\right)-\psi\left(\frac{3}{2}-n\right)+\ln\left(\lambda\right)+\pi i\right)\qquad |\lambda|>1
\end{align}
And the Meijers G function have the following integral representation( some basic property about Meijer's G function are included in \cite{BeukerMeijersG}):
\begin{align}
G^{2,0}_{2,2}\left(\lambda\right|\left.\begin{array}{cc}
	\frac{2}{3} & \frac{8}{3} \\
	\frac{7}{6} & -\frac{5}{6}
\end{array}\right)=\frac{1}{2\pi i}\int_L \frac{\Gamma\left(\frac{7}{6}+s\right)\Gamma\left(-\frac{5}{6}+s\right)}{\Gamma\left(\frac{2}{3}+s\right)\Gamma\left(\frac{8}{3}+s\right)}\lambda^{-s}ds
\end{align}
The poles are $s=\frac{5}{6}$, $s=\frac{-1}{6}$, $s=\frac{-7}{6}$,... on th left of contour $L$, pick up all the residues at these poles we have the following Taylor series within $|\lambda|<1$:
\begin{align}
&G^{2,0}_{2,2}\left(\lambda\right|\left.\begin{array}{cc}
	\frac{2}{3} & \frac{8}{3} \\
	\frac{7}{6} & -\frac{5}{6}
\end{array}\right)=\frac{16}{15\pi}\lambda^{-\frac{5}{6}}-\frac{4}{3\pi}\lambda^{\frac{1}{6}}+\frac{1}{\pi^2}\sum_{n\geq 0}\lambda^{\frac{7}{6}+n}\frac{\Gamma\left(n-\frac{1}{2}\right)\Gamma\left(\frac{3}{2}+n\right)}{n!\Gamma\left(n+3\right)}\left(A_n+A_{n+2}-\psi\left(\frac{3}{2}+n\right)\right.\notag\\
&\left.-\psi\left(\frac{3}{2}-n\right)-\ln\lambda\right)\qquad |\lambda|<1
\end{align}
And the integral representation will tell you that when $|\lambda|>1$, $G^{2,0}_{2,2}\left(\lambda\right|\left.\begin{array}{cc}
	\frac{2}{3} & \frac{8}{3} \\
	\frac{7}{6} & -\frac{5}{6}
\end{array}\right)=0$, but we can properly set:
\begin{align}\label{Gextension04}
	G^{2,0}_{2,2}\left(\lambda\right|\left.\begin{array}{cc}
		\frac{2}{3} & \frac{8}{3} \\
		\frac{7}{6} & -\frac{5}{6}
	\end{array}\right)=\lambda^{\frac{5}{6}} G^{2,0}_{2,2}\left(\frac{1}{\lambda}\right|\left.\begin{array}{cc}
	\frac{2}{3} & \frac{8}{3} \\
	\frac{7}{6} & -\frac{5}{6}
\end{array}\right)\qquad |\lambda|>1
\end{align}
For later covenience we normalize the solutions as:
\begin{align}
&\chi_0\left(\lambda\right)=\frac{1}{16\times 2^{\frac{2}{3}}}\left(1-\lambda\right)^{-\frac{5}{6}}\lambda^{\frac{7}{6}}{}_2F_1\left(\frac{3}{2},-\frac{1}{2};3;\lambda\right)
&\chi_{1}\left(\lambda\right)=\frac{1}{8\times 2^{\frac{2}{3}}}\left(1-\lambda\right)^{-\frac{5}{6}}G^{2,0}_{2,2}\left(\lambda\right|\left.\begin{array}{cc}
	\frac{2}{3} & \frac{8}{3} \\
	\frac{7}{6} & -\frac{5}{6}
\end{array}\right)
\end{align}
It is obvious that (when $|\lambda|<1$):
\begin{align}
\chi_0\left(e^{2\pi i}\lambda\right)=e^{\frac{7\pi i}{3}}\chi_0\left(\lambda\right)
\end{align}
By using the series expansion within $|\lambda|<1$, we can readily obtain:
\begin{align}
	\chi_1\left(e^{2\pi i}\lambda\right)=e^{\frac{\pi i}{3}}\chi_1\left(\lambda\right)+2i e^{\frac{\pi i}{3}}\chi_0\left(\lambda\right)
\end{align}
Therefore we have the monodromy around $0$:
\begin{align}
M_0=T^2=\left(\begin{array}{cc}
	e^{\frac{7\pi i}{3}} & o \\
	2e^{\frac{5\pi i}{6}} & e^{\frac{\pi i}{3}}
\end{array}\right)
\end{align}
About the $STS$ transformation, knowing ${}_2F_1\left(\frac{3}{2},\frac{-1}{2};3;\lambda\right)$'s behaviour when $|\lambda|<1$, we have:
\begin{align}
&\chi_0\left(\frac{1}{\lambda}\right)=\frac{1}{16\times 2^{2/3}}\left(1-\frac{1}{\lambda}\right)^{-\frac{5}{6}}\lambda^{-\frac{7}{6}}{}_2F_1\left(\frac{3}{2},\frac{-1}{2};3;1/\lambda\right)\notag\\
&=\frac{e^{\frac{-5\pi i}{6}}}{16\times 2^{2/3}}\left(1-\lambda\right)^{-\frac{5}{6}}\lambda^{-\frac{1}{3}}\left(2i\lambda^{\frac{1}{3}}G^{2,0}_{2,2}\left(\frac{1}{\lambda}\right|\left.\begin{array}{cc}
	\frac{2}{3} & \frac{8}{3} \\
	\frac{7}{6} & -\frac{5}{6}
\end{array}\right)+\lambda^{\frac{3}{2}}{}_2F_1\left(\frac{3}{2},-\frac{1}{2};3;\lambda\right)\right)\notag\\
&=e^{\frac{-\pi i}{3}}\chi_1\left(\lambda\right)+e^{-\frac{5\pi i}{6}}\chi_0\left(\lambda\right)\qquad |\lambda|<1
\end{align}
From the extension we choose \ref{Gextension04} we also have:
\begin{align}
\chi_1\left(\frac{1}{\lambda}\right)=-e^{\frac{\pi i}{6}}\chi_1\left(\lambda\right)\qquad |\lambda|<1
\end{align}
Therefore under $STS$ transformation we have:
\begin{align}
M_R=\left(\begin{array}{cc}
	-e^{\frac{\pi i}{6}}& -e^{\frac{2\pi i}{3}}\\
	0 & -e^{\frac{\pi i}{6}}
\end{array}\right)
\end{align}



\subsection{$\mathcal{N} = 4$}

In terms of $\Gamma(2)$ haupt function $\lambda(\tau)=\frac{\vartheta_2(\tau)^4}{\vartheta_3(\tau)^4}$, twisted LMDE \ref{MDE-weight-two-unflavored-N4} can be expressed as the following generalized hypergeometric equation\cite{Naculich:1989NuPhB.323..423N}:
\begin{align}
\left(D-\beta_1\right)\left(D-\beta_2\right)\chi(\lambda(\tau))-\lambda\left(D+1-\alpha_1\right)\left(D+1-\alpha_2\right)\chi(\lambda(\tau))=0
\end{align}
where $\alpha_1=\frac{1}{4}$, $\alpha_2=\frac{5}{4}$, $\beta_1=\frac{3}{4}$, $\beta_2=-\frac{1}{4}$, $D$ represents $\lambda\frac{d}{d\lambda}$. This equation admits the following two solutions near $\lambda=0$:
\begin{align}
&\chi_0(\lambda)=\frac{1}{8}\lambda^{3/4}\,{}_2F_1\left(\frac{3}{2},\frac{1}{2};2;\lambda\right)\\
&\chi_1(\lambda)=\pi G_{2,\,2}^{2,\,0} \left( {\begin{matrix}    {} & {1/4,5/4}  \cr    {- 1/4, 3/4\,} & {}  \cr  \end{matrix} \;\left| {\;\lambda} \right.} \right)=\frac{\pi}{2\pi i}\int_L\frac{\Gamma\left(s-\frac{1}{4}\right)\Gamma\left(\frac{3}{4}+s\right)}{\Gamma\left(s+\frac{1}{4}\right)\Gamma\left(\frac{5}{4}+s\right)}\lambda^{-s}ds
\end{align}
with $L$ as a contour at the right side of a sequence of poles $s=\frac{1}{4}$, $s=-\frac{3}{4}$, ..., $s=-n+\frac{1}{4}$.
\begin{tikzpicture}
\fill (0.25cm,0) circle (2pt) node[below]{\tiny $\frac{1}{4}$};
\fill (-0.75cm,0) circle (2pt) node[below]{\tiny $-\frac{3}{4}$};
\fill (-1.75cm,0) circle (2pt) node[below]{\tiny $-\frac{7}{4}$};
\fill (-2.75cm,0) circle (2pt) node[below]{\tiny $-\frac{11}{4}$};
\draw [->](-3cm,0)--(3cm,0);
\draw [->](0,-2cm)--(0,2cm);
\draw [red,thick,->](0.5cm,-2cm)--(0.5cm,2cm) 
node[near start]{$L$};
\end{tikzpicture}

 We can easily get series expression of $\chi_1$ converging within the unit disk $0<|\lambda|<1$ by picking up the residues mentioned previously:
\begin{align}
&\chi_1(\lambda)=\frac{2}{\lambda^{1/4}}+\frac{\lambda^{3/4}}{\pi}\sum_{n=0}^{\infty}\frac{\Gamma\left(\frac{3}{2}+n\right)\Gamma\left(\frac{1}{2}+n\right)}{n!\Gamma\left(n+2\right)}\left(-\psi\left(-n-\frac{1}{2}\right)-\psi\left(\frac{1}{2}-n\right)-\ln \lambda+A_n+A_{n+1}\right)\lambda^{n}\notag\\
&=\frac{2}{\lambda^{1/4}}-4\ln \lambda \chi_0(\lambda)-\frac{1}{2}\sum_{n=0}^{\infty}\frac{\left(\frac{3}{2}\right)_n\left(\frac{1}{2}\right)_n}{n!\left(2\right)_n}\left(\psi\left(-n-\frac{1}{2}\right)+\psi\left(\frac{1}{2}-n\right)-A_n-A_{n+1}\right)\lambda^{n+3/4} 
\end{align}
where $A_n$ is the following:
\begin{align}
A_n=-\gamma+\frac{1}{1}+\frac{1}{2}+\frac{1}{3}+...+\frac{1}{n}
\end{align}
It is worth noting that:
\begin{align}
	& G_{2,\,2}^{2,\,0} \left( {\begin{matrix}
			{} & {a,a + 1}  \cr    {a - 1/2,a + 1/2\,} & {}  \cr  \end{matrix} \;\left| {\;z} \right.} \right) =   \cr 
	&  = {2 \over \pi }\theta \left( {1 - \left| z \right|} \right)z^{a - {1 \over 2}} E\left( {1 - z} \right)
	\quad \left| {\;z \notin \left( { - 1,0} \right)} \right.
\end{align}
which means that within the unit disk $\chi_1(\lambda)=2\lambda^{-\frac{1}{4}}E(1-\lambda)$ when $\lambda\notin \left(-1,0\right)$. $E$ represents the Elliptic E function. It is natural that monodromy matrix around $0$ is:
\begin{align}
M_0=\left(
\begin{matrix}
	&-i   &0\\
	&8\pi &-i
\end{matrix}
\right)
\end{align}
Using another base:
\begin{align}
\left(\begin{array}{c}
	\operatorname{ch}_0\\
	\operatorname{ch}_1
\end{array}\right)=\left(\begin{array}{cc}
1 & 0\\                                                          
1 & \frac{1}{4\pi i}
\end{array}\right)\left(\begin{array}{c}
\chi_0\\
\chi_1
\end{array}\right)
\end{align}
we can obtain $T^2$ matrix under bases $\operatorname{ch}_0$ and $\operatorname{ch}_1$:
\begin{align}
M_0^{\prime}=T^2=\left(
\begin{array}{cc}
	-i & 0\\
	-2i & -i\\
\end{array}\right)
\end{align}
We can also compute the STS transformation matrix. Observing that acting STS on $\tau$ is equivalent to transforming $\lambda$ to $\frac{1}{\lambda}$, we believe that $\chi_0\left(\frac{1}{\lambda}\right)$ and $\chi_{1}\left(\frac{1}{\lambda}\right)$ are also solutions to this hypergeometric equation. Therefore they should be linear combinations of $\chi_0(\lambda)$ and $\chi_1(\lambda)$. We can determine the coefficient of linear combinations by looking at $\chi_0\left(\frac{1}{\lambda}\right)$ and $\chi_1\left(\frac{1}{\lambda}\right)$'s behaviours near $\lambda=0$ and $\lambda=\infty$. For $\chi_0\left(\frac{1}{\lambda}\right)$, if we want to determine its behaviour around $\lambda=0$, we need to know the analytic continuation to $\infty$ of $\chi_0\left(\lambda\right)$. In fact, for ${}_{2}F_{1}\left(\frac{3}{2},\frac{1}{2};2,\lambda\right)$, it has the following integral representation:
\begin{align}
{}_2 F_1\left(\frac{3}{2},\frac{1}{2};2,\lambda\right)=\frac{\Gamma\left(2\right)}{\Gamma\left(\frac{3}{2}\right)\Gamma\left(\frac{1}{2}\right)}\frac{1}{2\pi i}\int_L \frac{\Gamma\left(s+\frac{3}{2}\right)\Gamma\left(s+\frac{1}{2}\right)\Gamma\left(-s\right)}{\Gamma\left(s+2\right)}\left(-\lambda\right)^s ds
\end{align}
The contour $L$ is depicted as follows:
\begin{tikzpicture}
	\fill (-0.5cm,0) circle (2pt) node[below]{\tiny $-\frac{1}{2}$};
	\fill (-1.5cm,0) circle (2pt) node[below]{\tiny $-\frac{3}{2}$};
	\fill (-2.5cm,0) circle (2pt) node[below]{\tiny $-\frac{5}{2}$};
	\fill (0,0) circle (2pt) node[below]{\tiny $0$};
		\fill (1cm,0) circle (2pt) node[below]{\tiny $1$};
		\fill (2cm,0) circle (2pt) node[below]{\tiny $2$};
	\draw [->](-3cm,0)--(3cm,0);
	\draw [->](0,-2cm)--(0,2cm);
	\draw [red,thick,->](-0.25cm,-2cm)--(-0.25cm,2cm) 
	node[near start]{$L$};
\end{tikzpicture}
To study the behaviour when $|\lambda|<1$, we simply pick up the residues of the poles on the right hand side:
\begin{align}
&{}_2 F_1\left(\frac{3}{2},\frac{1}{2};2,\lambda\right)=\frac{\Gamma\left(2\right)}{\Gamma\left(\frac{3}{2}\right)\Gamma\left(\frac{1}{2}\right)}\sum_{n\geq 0}\operatorname{Res}_{s=n}\left(\frac{\Gamma\left(s+\frac{3}{2}\right)\Gamma\left(s+\frac{1}{2}\right)\Gamma\left(-s\right)}{\Gamma\left(s+2\right)}\left(-\lambda\right)^s\right)\\
&=\frac{\Gamma\left(2\right)}{\Gamma\left(\frac{3}{2}\right)\Gamma\left(\frac{1}{2}\right)}\sum_{n\geq 0}\frac{\left(-\right)^n}{n!}\frac{\Gamma\left(n+\frac{3}{2}\right)\Gamma\left(n+\frac{1}{2}\right)}{\Gamma\left(n+2\right)}\left(-\lambda\right)^n=\sum_{n\geq 0}\frac{\left(\frac{3}{2}\right)_n\left(\frac{1}{2}\right)_n}{n!\left(2\right)_n}\lambda^n\qquad \left|\lambda\right|<1
\end{align}
For $\left|\lambda\right|>1$, we can study its Laurent expansion by picking up the residues on the left hand side of the contour $L$:
\begin{align}
&{}_2 F_1\left(\frac{3}{2},\frac{1}{2};2;\lambda\right)=\frac{2}{\pi}\sum_{n\geq 0}\operatorname{Res}_{s=-n-\frac{1}{2}}\left(\frac{\Gamma\left(s+\frac{3}{2}\right)\Gamma\left(s+\frac{1}{2}\right)\Gamma\left(-s\right)}{\Gamma\left(s+2\right)}\left(-\lambda\right)^s\right)\notag\\
&=\frac{2}{\pi}\sum_{n\geq 0}\frac{\left(-\right)^{n+1}\Gamma\left(n+\frac{3}{2}\right)\Gamma\left(n+\frac{1}{2}\right)}{\pi n! \left(n+1\right)!}\left(-\lambda\right)^{-n-\frac{3}{2}}\left(-\psi\left(n+\frac{3}{2}\right)-\psi\left(-n+\frac{1}{2}\right)+\ln\left(-\lambda\right)+A_n+A_{n+1}\right)\notag\\
&+\frac{4}{\pi}\left(-\lambda\right)^{-\frac{1}{2}}\qquad \left|\lambda\right|>1
\end{align}
Take $(-)^{-\frac{1}{2}}=-i$, and $\ln\left(-\lambda\right)=\ln\lambda+\pi i$, and note that $\psi\left(-n-\frac{1}{2}\right)=\psi\left(n+\frac{3}{2}\right)$. Then for $\left|\lambda\right|<1$, we have:
\begin{align}
\chi_0\left(\frac{1}{\lambda}\right)=\frac{-i}{4\pi}\chi_1\left(\lambda\right)+\chi_0\left(\lambda\right)\qquad \left|\lambda\right|<1
\end{align}
And we also have:
\begin{align}
\chi_1\left(\frac{1}{\lambda}\right)=\chi_1\left(\lambda\right)(???)
\end{align}
Therefore we can obtain:
\begin{align}
M_R=\left(\begin{array}{cc}
	1 & \frac{-i}{4\pi} \\
	0 & 1\\
\end{array}\right)
\end{align}
In the $\operatorname{ch}_0\left(\lambda\right)$ and $\operatorname{ch}_1\left(\lambda\right)$ bases, it can be recasted as:
\begin{align}
M_R^{\prime}=\left(\begin{array}{cc}
	0 & 1 \\
	-1 & 2\\
\end{array}\right)
\end{align}

\subsection{$\mathcal{T}_{1,2}$}
The $\mathcal{T}_{1,2}$ in the unflavored limit actually obeys a six order untwisted modular differential equation:
\begin{align}
\left(D_q^{(3)}-220 E_4D_q^{(1)}+700 E_6\right)\mathcal{I}_{1,2}=0
\end{align}
Rewrite the equation in terms of the reciprocal of Klein-J invariant $K(q)=\frac{1}{j(q)}$, we can recast this equation as the following:
\begin{align}
\left(\prod_{i=1}^{3}\left(D_K+\beta_i-1\right)-K\prod_{i=1}^{3}\left(D_K+\alpha_i\right)\right)\chi(K)=0	
\end{align} 
Where $\alpha=0,\frac{1}{3},\frac{2}{3}$, $\beta=\frac{1}{6}, \frac{7}{6}, \frac{7}{6}$, and $D_K$ represents $K\frac{d}{dK}$. We choose to compute the S and T matrix under the following bases, which comes from the $\mathcal{T}_{1,2}$ Schur index and its modular transformation partners:
$$\operatorname{ch}_0\qquad \operatorname{ch}_{\log,1}\qquad \operatorname{ch}_{\log,2}$$
They can be expressed as a linear combinations of the three linear independent series below:
\begin{align}
&\chi_0(K)=K^{5/6}{}_3 F_2\left(\frac{5}{6}, \frac{7}{6}, \frac{3}{2}; K\right)\\
&\chi_1(K)=\frac{-12\pi^{3/2}}{K^{1/6}}+\sum_{n=0}^{\infty}K^{5/6+n}\frac{\Gamma\left(\frac{5}{6}+n\right)\Gamma\left(\frac{7}{6}+n\right)\Gamma\left(\frac{3}{2}+n\right)}{n!\left(n+2\right)!\left(n+2\right)!}\left(\psi\left(\frac{5}{6}+n\right)+\psi\left(\frac{7}{6}+n\right)+\psi\left(\frac{3}{2}+n\right)+\ln K-A_n-2 A_{n+1}\right)\\
&\chi_2(K)=\frac{12\pi^{3/2}}{K^{1/6}}\left(6-3\ln 12+\ln K\right)+\sum_{n=0}^{\infty}K^{\frac{5}{6}+n}\frac{\Gamma\left(\frac{5}{6}+n\right)\Gamma\left(\frac{7}{6}+n\right)\Gamma\left(\frac{3}{2}+n\right)}{n!\left(n+2\right)!\left(n+2\right)!}\left(-\frac{1}{2}\left(\psi\left(\frac{5}{6}+n\right)+\psi\left(\frac{7}{6}+n\right)+\psi\left(\frac{3}{2}+n\right)+\ln K\right)^2-\frac{1}{2}\psi^{\prime}\left(\frac{5}{6}+n\right)-\frac{1}{2}\psi^{\prime}\left(\frac{7}{6}+n\right)-\frac{1}{2}\psi^{\prime}\left(\frac{3}{2}+n\right)+\left(A_n+2A_{n+1}\left(\right)\right)\left(\psi\left(\frac{5}{6}+n\right)+\psi\left(\frac{7}{6}+n\right)+\psi\left(\frac{3}{2}+n\right)+\ln K\right)-2A_n A_{n+1}-A_{n+1}^2-B_n-2B_{n+1}\right)
\end{align}
And we can obtain the following relations:
\begin{align}
\operatorname{ch}_0=a\chi_0\qquad \operatorname{ch}_1=b\chi_1\qquad \operatorname{ch}_2=c\chi_2-\frac{5}{4}d\chi_0
\end{align}
where $a=\frac{1}{48\sqrt{3}\pi^{3/2}}$, $b=\frac{-i}{48\sqrt{3}\pi^{5/2}}$, $c=\frac{-1}{96\sqrt{3}\pi^{7/2}}$, $d=\frac{1}{48\sqrt{3}\pi^{3/2}}$. Note that the monodromy matrices around $0$ and $1$, which can be refered to T and S transformation respectively, are computed as:
\begin{align}
M_0=\left(
\begin{array}{ccc}
	0 & 1 & 0 \\
	0 & 0 & 1 \\
	-1 & 3 \sqrt[3]{-1} & -3 (-1)^{2/3} \\
\end{array}
\right)
\quad 
M_1=\left(
\begin{array}{ccc}
	-1 & 3 \sqrt[3]{-1} & -3 (-1)^{2/3} \\
	0 & 1 & 0 \\
	0 & 0 & 1 \\
\end{array}
\right)
\end{align}
under the Meilin-Barnes bases \cite{molag:2015monodromy}:
\begin{align}
	I_j(K)=\frac{(-1)^3}{\left(2\pi i\right)^3}\int_L\left(\prod_{i=1}^{3}\Gamma\left(\alpha_i+s\right)\Gamma\left(1-\beta_i-s\right)\right)e^{-3\pi i+2n\pi i}ds
\end{align}
for $j=0,1,2$. In fact we can easily find that:
\begin{align}
&I_0(K)=-\frac{i\left(9\pi^2\chi_0(K)+6i\pi\chi_1(K)+2\chi_2(K)\right)}{8\pi^2}\notag\\
&I_1(K)=-\frac{(-1)^{1/6}\left(\pi^2\chi_0(K)+2i\pi\chi_1(K)+2\chi_2(K)\right)}{8\pi^2}\notag\\
&I_2(K)=\frac{(-1)^{1/3}\left(i\pi^2\chi_0(K)+2\pi\chi_1(K)+2i\chi_2(K)\right)}{8\pi^2}\notag
\end{align}
Therefore we can obtain the monodromy matrix around 0 and 1 under the bases $\operatorname{ch}_0$, $\operatorname{ch}_{1,\log}$, $\operatorname{ch}_{2,\log}$ after suitable conjugation:
\begin{align}
T=M_0^{\prime}=\left(
\begin{array}{ccc}
	-(-1)^{2/3} & 0 & 0 \\
	-2 (-1)^{2/3} & -(-1)^{2/3} & 0 \\
	(-1)^{2/3} & (-1)^{2/3} & -(-1)^{2/3} \\
\end{array}
\right)\qquad
S=M_1^{\prime}=\left(
\begin{array}{ccc}
	0 & 0 & 1 \\
	0 & 1 & 0 \\
	1 & 0 & 0 \\
\end{array}
\right)
\end{align}

